Text-Guided Image Clustering

Image clustering divides a collection of images into meaningful groups, typically interpreted post-hoc via human-given annotations. Those are usually in the form of text, begging the question of using text as an abstraction for image clustering. Current image clustering methods, however, neglect the use of generated textual descriptions. We, therefore, propose Text-Guided Image Clustering, i.e., generating text using image captioning and visual question-answering (VQA) models and subsequently clustering the generated text. Further, we introduce a novel approach to inject task- or domain knowledge for clustering by prompting VQA models. Across eight diverse image clustering datasets, our results show that the obtained text representations often outperform image features. Additionally, we propose a counting-based cluster explainability method. Our evaluations show that the derived keyword-based explanations describe clusters better than the respective cluster accuracy suggests. Overall, this research challenges traditional approaches and paves the way for a paradigm shift in image clustering, using generated text.

==> aux/methods.tex <==
\begin{table*}[h]
\small
    \centering
    \begin{tabular}{llllllll}
\toprule
 method &        stl10 & fashion\_mnist &     cifar100 &   imagenet10 &      cifar10 & tiny\_imagenet & Avg \\
\midrule
\textbf{Embeddings} & & & & & & & \\
 flamingo visual &   95.4 / 95.78 &  58.77 / 58.66 &  47.82 / 44.03 &  98.92 / 99.65 &   83.75 / 83.0 &   70.46 / 57.2 &  75.85 / 73.05\\
 flamingo sbert &   94.2 / 97.45 &   50.6 / 54.38 &  58.18 / 58.13 &   95.2 / 97.85 &  85.51 / 93.28 &   62.47 / 48.3 & 74.36 / 74.90\\
\hline
\textbf{Baselines} & & & & & & & \\
cc & 76.4 / 85.0 & 0 / 0 & 43.1 / 42.9 & 85.9 / 89.3 & 70.5 / 79.0 & 34.0 / 14.0 & \\
SOTA papWcode &  86.0 / 92.9 & 76.7 / 85.6 & 58.3 / 58.4 & 92.7 / 96.9 &  85.0 / 91.8 & 	44.9 / 30.5 & \\
\hline
\textbf{Ours} & & & & & & & \\
Text Emb. init & & & & & & & \\
cc+text & 0 / 0 & 0 / 0 & 62.5 / 56.02 & 96.78 / 98.83 & 92.66 / 97.03 & 37.83 / 11.79 & \\
Mult. text sup. & 94.89 / 97.76 & 0 / 0 & 62.93 / 56.87 & 94.66 / 97.72 & 87.19 / 92.44 & 0 / 0 & \\
\bottomrule
\end{tabular}
    \caption{GIT Clustering quality, encoder vs. SBERT, (NMI / Accuracy)}
    \label{tab:git_visual_vs_sbert}
\end{table*}

==> aux/old/abstract.tex <==
\begin{abstract}

Common to other fields in machine learning, clustering benefits from scaling models and data, especially using pre-trained foundation models. 
These large models allow to navigate between modalities. 
%TODO: Next sentence much better
We argue that a textual description often captures the semantics of what we want to cluster better.
In this work, we investigate how we can use generated text for image clustering.
We observe that clustering the text representation obtained by image-to-text models often achieves competitive performance.
Furthermore, we introduce "zero-shot clustering" to guide the text generation process and provide experiments on how this improves clustering performance.
Existing literature proved that multi-modal clustering improves clustering performance. We extend this claim by showing that multi-modal models using noisily generated texts also improve clustering performance.
Finally, we provide a case study where we create a textual description for each cluster, establishing explainability in the natural form of text.
In summary, we make the case that text clustering obtains good clustering performance, improves consistency with human clustering understanding and provides the possibility to describe clusters.
\end{abstract}

==> aux/old/caption_analysis.tex <==
\section{Dedicated VQA}


Overview over all asked questions

==> aux/old/dedicated_vqa_max.tex <==
\begin{table}%[h]
\resizebox{.5\textwidth}{!}{%

\begin{tabular}{c|cc|cc|cc}
\toprule
{} & \multicolumn{2}{c}{ViT} & \multicolumn{2}{c}{TF-IDF} & \multicolumn{2}{c}{SBERT} \\
{} &    NMI &    nmi &    NMI &    nmi &    NMI &    nmi \\
\midrule
FER2013                  &  36.81 &  21.23 &  48.47 &  29.63 &  48.30 &  34.92 \\
LSUN                     &  61.40 &  64.22 &  68.81 &  66.26 &  73.54 &  74.87 \\
Human Action Recognition &  48.80 &  44.86 &  49.16 &  45.32 &  57.12 &  51.35 \\
Sports10                 &  82.77 &  87.68 &  87.93 &  93.90 &  87.19 &  91.94 \\
iNaturalist2021          &  41.88 &  60.61 &  41.92 &  42.75 &  46.73 &  59.61 \\
Places365                &  31.78 &  61.13 &  27.10 &  56.18 &  29.44 &  59.52 \\
\bottomrule
\end{tabular}
}
\caption{Zero-Shot Clustering performance (e.g. "Which activity is performed"), comparing the visual encoder (ViT) to Tf-IDF and SBERT, showing best performing Question}
\label{tab:ded_vqa_max}
\end{table}

==> aux/old/dedicated_vqa_mean.tex <==
\begin{table}%[h]
\resizebox{.5\textwidth}{!}{%

\begin{tabular}{c|cc|cc|cc}
\toprule
{} & \multicolumn{2}{c}{ViT} & \multicolumn{2}{c}{TF-IDF} & \multicolumn{2}{c}{SBERT} \\
{} &    acc &    nmi &    acc &    nmi &    acc &    nmi \\
\midrule
FER2013                  &  36.81 &  21.23 &  42.31 &  22.14 &  43.05 &  27.26 \\
LSUN                     &  61.40 &  64.22 &  58.81 &  55.48 &  64.79 &  62.16 \\
Human Action Recognition &  48.80 &  44.86 &  45.77 &  40.81 &  52.72 &  47.13 \\
Sports10                 &  82.77 &  87.68 &  83.77 &  89.98 &  86.20 &  91.50 \\
iNaturalist2021          &  41.88 &  60.61 &  36.45 &  33.88 &  45.33 &  55.56 \\
Places365                &  31.78 &  61.13 &  21.35 &  49.94 &  23.96 &  54.32 \\
\bottomrule
\end{tabular}
}
\caption{Zero-Shot Clustering performance (e.g. "Which activity is performed"), comparing the visual encoder (ViT) to Tf-IDF and SBERT, showing average performance}
\label{tab:ded_vqa_mean}
\end{table}

==> aux/old/dedicated_vqa_performance.tex <==

\begin{table}%[h]
\resizebox{.48\textwidth}{!}{%

\begin{tabular}{cc|cccc|cc|cc}
\toprule
     &       & \multicolumn{2}{c}{Image} & \multicolumn{2}{c}{Keywords} & \multicolumn{2}{c}{Inertia} & \multicolumn{2}{c}{Silhouette} \\
     &       &   Acc &   NMI &      Acc &   NMI &            Acc &            NMI &            Acc &            NMI \\
Dataset & Representation &       &       &          &       &                &                &                &                \\
\midrule
Sports10 & TF-IDF &  0.91 &  0.92 &     0.99 &  0.97 &                       0.85 &           \underline{0.94} &                       0.85 &           \underline{0.94} \\
        & SBERT &  0.91 &  0.92 &     0.99 &  0.97 &           \underline{0.99} &  \underline{\textbf{0.98}} &           \underline{0.99} &  \underline{\textbf{0.98}} \\
iNaturalist2021 & TF-IDF &  0.43 &  0.62 &     0.42 &  0.48 &                       0.33 &                       0.44 &                       0.33 &                       0.44 \\
        & SBERT &  0.43 &  0.62 &     0.50 &  0.59 &           \underline{0.44} &               \textbf{0.6} &                       0.42 &                       0.58 \\
LSUN & TF-IDF &  0.63 &  0.67 &     0.76 &  0.69 &                       0.63 &                       0.56 &           \underline{0.69} &                       0.66 \\
        & SBERT &  0.63 &  0.67 &     0.68 &  0.69 &  \underline{\textbf{0.75}} &                       0.63 &  \underline{\textbf{0.81}} &  \underline{\textbf{0.74}} \\
HAR & TF-IDF &  0.51 &  0.46 &     0.51 &  0.45 &                        0.5 &              \textbf{0.46} &                        0.5 &              \textbf{0.46} \\
        & SBERT &  0.51 &  0.46 &     0.55 &  0.48 &  \underline{\textbf{0.61}} &  \underline{\textbf{0.53}} &  \underline{\textbf{0.61}} &  \underline{\textbf{0.53}} \\
FER2013 & TF-IDF &  0.36 &  0.21 &     0.44 &  0.26 &   \underline{\textbf{0.5}} &  \underline{\textbf{0.31}} &   \underline{\textbf{0.5}} &  \underline{\textbf{0.31}} \\
        & SBERT &  0.36 &  0.21 &     0.46 &  0.28 &           \underline{0.46} &  \underline{\textbf{0.35}} &   \underline{\textbf{0.5}} &  \underline{\textbf{0.38}} \\
\bottomrule
\end{tabular}

}
\caption{Zero-Shot Clustering performance. By inertia and silhouette score, the best of 4 prompt-guided clusterings is chosen, e.g. "Which activity is performed". Bold numbers are better than keyword performance, underlined better than image representations.}
\label{tab:ded_vqa_performance}
\end{table}

==> aux/old/explainability_for_improving.tex <==
\section{Can explainability enhance clustering performance?}


Now we obtained a description for each cluster. 
Apart from improved explainability, we ask the question of whether the cluster descriptions can support clustering performance.

\textbf{Setup.} Therefore we treat the descriptions as centroids in a combined text-image. We use the publicly available CLIP %TODO cite, clip version HF
checkpoint to obtain the representations for each image and the cluster descriptions.
Here we compare with 
\begin{itemize}
    \item K-Means clustering on Image space
    \item Zero-shot learning wrt. to cluster label names
    \item Zero-Shot learning with respect XAI descriptions obtained by the ground truth
    \item Zero-Shot learning with respect to XAI descriptions obtained by the predicitons
    \item (Maybe: By kmenas with centroid 
\end{itemize}


\textbf{Results.} 
\begin{itemize}
    \item It's clear that 2 serves as upper bound for 3 and 3 as upper bound for 2
    \item That spectrum is often very clear. Some loss due to summarization
    \item We see improvement across the board 
    \item Discussion: Dedicated methods should improve 
\end{itemize} 



==> aux/old/related_work_old_01_06_2023.tex <==
\section{Related Work}

GOAL: Beschreibung des related works, sodass die Frage aufkommt: "Warum hat noch niemand den generierten Text für Clustering genutzt"?

\textbf{Deep Clustering.} 

TODO: @Luki, bitte hier relativ kurz was dazu schreiben
DEC; IDec, whatever is used in Experiments

- From clustering to deep clustering
- Methods like DEC, IDEC; Contr. Clust. and follow-up work such as TCL
- Multi-View Clustering

\textbf{Descriptive Clustering.} 
A separate stream of research is descriptive clustering. %TODO citation
\begin{itemize}
    \item Descriptive Clustering
\end{itemize}



\textbf{Image-Text Models.}

% @Kevin: Add your findings here
% Note: It should naturally to the usage of Blip2
Image captioning is the task concerned with generating a textual description of an image.

- datasets: scraped / labeled / filtered
- models: flamingo / blip etc.


Image -> Text
\begin{itemize}
    \item Flamingo Mini: Trained on Conceptual Captions
    \item Harvested from Internet and hypernymization 
    \item Nothing manually labeled 
\end{itemize}


\textbf{Image Clustering.}


\textbf{Text Clustering.}


\textbf{Multi-Modal Clustering.}
% Ziel: Multi-View Clustering exkludieren. Evtl nur in der Discussion erwähnen.
%TODO - Lukas: Views sind unabhängig generiert z.B. Vase einmal von Kamera fotographiert und einmal von LIDAR abgetastet.
The idea of using visual and textual features to solve language and vision tasks is not new \cite{agrawal2007}. Different works have been utilizing surrounding contexts from web pages, scientific papers, and other forms of documents to cluster images accordingly \cite{x,y}.

What is new, are emerging LLMs and foundation models capable of describing images accurately. Although the image captioning capabilities of models have improved significantly over the last few years \cite{x,y}, there has been little research on its implications for image clustering.

Most multi-modal methods focus on learning encodings of texts that are attached to images. JECL \cite{yang2021jecl} trains parallel encoders and learns a joint target distribution from the image encoder and text encoder. \citet{xu2022} learns common semantics in high-level features by combining encoder representations of multiple modalities through feature networks. EAMC \cite{zhou2020end} introduces a divergence-based clustering objective to learn different modalities using adversarial fusion, and DM2C \cite{jiang2019dm2c} waives the assumption that pairing information of different modalities is available using a unified adversarial representation learning. 
Other methods enrich the semantic understanding of images with text \cite{cai2022semantic}, learn relationships between image and text \cite{jin2015cross, chaudhary2019novel}, or combine similar modalities into groups \cite{Chang2017, wang2020icmsc}.

So far, only \citet{Kong2022} use CLIP to generate text centroids assigned by the image features but image and text share the feature space and perform clustering on the shared encoder representations. They do not derive a textual representation for further reasoning.

% Connect it back to our work and what we do differently and why.

==> aux/old/single_answer_vqa.tex <==
\begin{table*}
    \centering
    \resizebox{.6\textwidth}{!}{
\begin{tabular}{lrrr}
\toprule
 & visual & tfidf & sbert \\
\midrule
lsun & 63.56 & 57.47 & 63.84 \\
sports10 & 90.16 & 83.84 & 95.61 \\
human\_action\_recognition & 53.44 & 48.92 & 56.42 \\
fer2013 & 32.72 & 38.63 & 42.56 \\
mean & 59.97 & 57.21 & 64.61 \\
\bottomrule
\end{tabular}

}
    \caption{Single answer VQA: "Which activity describes the image?". 4 prompts per dataset. Averaged performance of prompts }
    \label{tab:single_vqa_mean}
\end{table*}

\begin{table*}
    \centering
    \resizebox{.6\textwidth}{!}{
\begin{tabular}{lrrr}
\toprule
 & visual & tfidf & sbert \\
\midrule
lsun & 63.56 & 76.16 & 76.29 \\
sports10 & 90.16 & 84.23 & 97.80 \\
human\_action\_recognition & 53.44 & 50.04 & 58.33 \\
fer2013 & 32.72 & 39.24 & 43.90 \\
mean & 59.97 & 62.42 & 69.08 \\
\bottomrule
\end{tabular}

}
    \caption{Single answer VQA: "Which activity describes the image?". 4 prompts per dataset. Performance of best prompt per dataset }
    \label{tab:single_vqa_max}
\end{table*}

==> aux/old/tables/intro_pro_con_table.tex <==
% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{lll}
%     \toprule
% Representation & Pros & Cons \\
% \midrule
% Image &  full information &   no choice by relevance  \\
% &  &   non-important information for humans (background) \\
% &  &  spurious features \\
% Text &  small relevant features &   loss of information ("Rundungsfehler") \\
% &  interpretability &   captioning wrong \\
% \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}


\begin{table}%[h]
    \centering
    \resizebox{.45\textwidth}{!}{
    \begin{tabular}{lcc}
    \toprule
 & Image & Text \\
\midrule
Full information & \cmark &  \xmark \\
Abstraction & \xmark & \cmark \\
Dense information & \xmark & \cmark \\
Interpretability & \xmark & \cmark \\
Spurious features & Background & Wrong Text  \\ 
\bottomrule
    \end{tabular}
    }
    \caption{Comparison of properties of images and text.}
    \label{tab:pro_con}
\end{table}

==> aux/old/text_vs_latent_flamingo.tex <==
\begin{table*}[h]
\small
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{llllllll}
\toprule
 method &        stl10 & fashion\_mnist &     cifar100 &   imagenet10 &      cifar10 & tiny\_imagenet & Avg \\
\midrule
 flamingo visual &   95.4 / 95.78 &  58.77 / 58.66 &  47.82 / 44.03 &  98.92 / 99.65 &   83.75 / 83.0 &   70.46 / 57.2 &  75.85 / 73.05\\
 flamingo sbert &   94.2 / 97.45 &   50.6 / 54.38 &  58.18 / 58.13 &   95.2 / 97.85 &  85.51 / 93.28 &   62.47 / 48.3 & 74.36 / 74.90\\
 git visual &  92.58 / 94.08 &  58.04 / 57.84 &   48.1 / 43.76 &  97.57 / 99.02 &  73.41 / 79.98 &   61.11 / 43.7 & 71.80 / 69.73 \\
 git sbert &  93.95 / 97.36 &  51.71 / 53.19 &  51.78 / 53.29 &   96.16 / 98.2 &  78.97 / 88.93 &  57.26 / 41.94 & 71.64 / 72.15 \\
\bottomrule
\end{tabular}%
}
    \caption{clustering quality, visual encoder vs. SBERT, (NMI / Accuracy)}
    \label{tab:flamingo_visual_vs_sbert}
\end{table*}

==> aux/old/text_vs_latent_git.tex <==
\begin{table}
    \centering
    \resizebox{.5\textwidth}{!}{
\begin{tabular}{lllllll}
\toprule
 method &        stl10 & fashion\_mnist &     cifar100 &   imagenet10 &      cifar10 & tiny\_imagenet \\
\midrule
 visual &  0.93 / 0.94 &   0.58 / 0.58 &  0.48 / 0.44 &  0.98 / 0.99 &   0.73 / 0.8 &   0.61 / 0.44 \\
  sbert &  0.94 / 0.97 &   0.52 / 0.53 &  0.52 / 0.53 &  0.96 / 0.98 &  0.79 / 0.89 &   0.57 / 0.42 \\
  tfidf &  0.76 / 0.81 &   0.45 / 0.46 &  0.33 / 0.32 &  0.83 / 0.86 &  0.69 / 0.77 &    0.5 / 0.34 \\
\bottomrule
\end{tabular}
}
    \caption{GIT Clustering quality, encoder vs. SBERT, (NMI / Accuracy)}
    \label{tab:git_visual_vs_sbert}
\end{table}

==> aux/old/vqa.tex <==
\subsection{Keyword-Guided Clustering: Inserting Task Knowledge}
\label{subsec:keywords}

% Main message: Wir können die Textgenierung auf den Task Image Clustering generell zuschneiden

Previously, we have seen investigated the clustering performance of text generated using image captioning models.
As a logical next step, we ask the research question of how to generate text that is better suited for clustering. 
By using modern visual question-answering (VQA) models, it is possible to elicit dedicated information from images.

Given that it is common to (verbally) describe clusters using keywords, we hypothesize that it is beneficial to prompt the model to generate keywords.
This approach offers several advantages: 1) ground truth cluster names (as given by classification datasets) are typically described using keywords, 2) keywords provide useful inputs for simpler, traditional natural language processing methods such as TF-IDF, 3) keywords are useful for count-based analysis methods, such as the proposed cluster explainability algorithm in section \ref{subsec:explainability}.

\textbf{Setup. } 
%Based on the results of the last section, we use Blip-2 and sample 4 texts for each image. 
As it is the best model in Figure \ref{tab:captioning_results}, and text and image encoders are fixed, we use the Blip2 model. 
Additionally, during training Blip2, the text and image backbones are not fine-tuned with multi-modal data, improving the fairness of the comparison.
Based on the results depicted in Figure \ref{fig:num_captions}, we sample 5 texts for each image.
For each image, we generate text, using the Blip2 VQA model \footnote{https://huggingface.co/Salesforce/blip2-flan-t5-xl} with the prompt "Which keywords describe the image?".
%TODO: Will we add this
%Additionally, we provide a case study asking, how many should be created.

\input{aux/tables/keywords_vqa}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{aux/plots/num_kws_fig_sbert_accuracy.pdf}
%     \caption{An investigation of how many keywords are needed. The lines show the mean and standard error of the clustering accuracy of the SBERT representation.} %TODO: other plots in Appendix
%     \label{fig:num_kws}
% \end{figure}

\textbf{Results. } 
Table \ref{tab:keywords_vqa_main_table} compares the image backbone to the generated text and the generated keywords, named "Image", "Captions" and "Keywords" in the top column.
In general, we observe that Captions work best with Keywords achieving a very similar performance, where SBERT almost always outperforms TF-IDF.
On the other hand, images work well on datasets with a large number of ground truth classes and standard datasets. 
We believe this is due to the fact that the Blip2 image encoder is trained on ImageNet21k, supporting the clustering of STL10, Cifar10, and TinyImagenet. 
Importantly, we see that TF-IDF improves by 5\% on average by the creation of keywords. 
We interpret that such that the amount of generated information stays the same but it is more suitable for image clustering.


\subsection{Prompt-Guided Clustering: Inserting Domain Knowledge}
\label{subsec:zero-shot}

% Main message: Wir können die Textgeneriung auf spezielle Tasks "Facial Image Clustering " zuschneiden

% \input{aux/tables/dedicated_vqa_mean}
% \input{aux/tables/dedicated_vqa_max}

% \input{aux/tables/dedicated_vqa_example}

\begin{figure}
    \centering
    \includegraphics[width=.48\textwidth]{aux/plots/vqa_qualitative_change_new.pdf}
    \caption{Not soo big improvement in overall performance, but all room classes achieve confusion >= 80\%}
    \label{fig:vqa_qualitative_change}
\end{figure}

In real-world scenarios, typically, some domain knowledge about the given dataset is available. 
The ability of VQA models to retrieve dedicated information from images opens up the possibility to use this domain knowledge, using the natural form of text.
Note that this is not possible using standard image clustering models, nevertheless is very realistic.
An example is to ask "Which activity is performed in the picture?". 
In this work, we refer to this as \textit{Zero-Shot Clustering}.
Importantly, the task differs from typical zero-shot learning, as no information about quantity and types of classes is given. 

\textbf{Setup. } 
% Say why only these dataset
The questions were created by looking at the name of the dataset, and possibly looking for synonyms, e.g. for human action recognition "Which activity is performed?" is created. Find all questions in Appendix \ref{appdx:sec_ded_vqa}.

It is known that current language models possibly generate very different texts, even though the prompt seems similar to a human. 
Therefore we propose to use the two common clustering metrics (which need no labels), to decide which clustering is the best.
We use the K-Means loss, inertia, and silhouette score which takes inter- and intra-class distance into account.
The rest of the setup is the same as in keyword-guided image clustering, see section \ref{subsec:keywords}.
% How to choose best prompt: 
% - https://towardsdatascience.com/are-you-still-using-the-elbow-method-5d271b3063bd
% - https://scikit-learn.org/stable/modules/generated/sklearn.metrics.silhouette_score.html

% \input{aux/tables/dedicated_vqa_performance}

\textbf{Results. }
% Numbers improved; there is variance
In Figure \ref{fig:vqa_ded_questions} we observe that there is variance among multiple prompts, but we also observe that prompt-guided clustering achieves the best clustering.
This variance is a common phenomenon for prompting-based methods [CITE].
Using inertia as a proxy for finding the best prompt, Table \ref{tab:keywords_vqa_main_table} shows that, on average, prompt-guided image clustering performs best.



% - Inertia also manages to >= Img/Kw.

% - There is high standard deviation (Figure X)
% -> BUT This is a feature, because figure 5
%     - rooms are clustered perfectly well
%     - environment and scene best performance works well
%     - scene: dining + restaurant problems
%     - environments: tower church problematic

\begin{figure}[htb]
\centering
\includegraphics[width=0.48\textwidth]{aux/plots/scatter_performance.pdf}
\caption{Comparison of all prompts with previous BLIP2 representations.
We observe that dedicated questions can work well but are prone to large differences in performance}
\label{fig:vqa_ded_questions}
\end{figure}



==> aux/vqa_table.tex <==

\begin{table*}
    \centering
    \resizebox{.9\textwidth}{!}{
\begin{tabular}{lllllll}
\toprule
 & ViT backbone & caption\_tfidf & caption\_sbert & keywords\_visual & keywords\_tfidf & keywords\_sbert \\
dataset &  &  &  &  &  &  \\
\midrule
lsun & 63.56 & 74.15 & 84.36 & 63.56 & 75.05 & 68.93 \\
dtd & 55.52 & 42.42 & 47.86 & 55.52 & 42.02 & 48.18 \\
human\_action\_recognition & 53.44 & 48.43 & 47.14 & 53.44 & 49.85 & 53.87 \\
fer2013 & 32.72 & 25.02 & 29.07 & 32.72 & 39.17 & 39.69 \\
places365\_val\_subset & 32.24 & 26.60 & 29.42 & 32.24 & 26.88 & 28.53 \\
stl10 & 99.72 & 79.62 & 98.47 & 99.72 & 86.26 & 95.73 \\
imagenet10 & 99.80 & 89.63 & 92.50 & 99.80 & 91.34 & 98.22 \\
cifar10 & 99.25 & 86.01 & 97.41 & 99.25 & 93.10 & 97.26 \\
tiny\_imagenet & 73.25 & 53.90 & 61.86 & 73.25 & 56.13 & 60.79 \\
sports10 & 90.16 & 98.59 & 98.73 & 90.16 & 97.66 & 97.35 \\
inaturalist\_val\_subset & 69.30 & 51.98 & 64.07 & 69.30 & 57.65 & 61.22 \\
avg & 69.90 & 61.49 & 68.26 & 69.90 & 65.01 & 68.16 \\
\bottomrule
\end{tabular}

}
    \caption{Caption vs general VQA: "Which keywords describe the image?" => Tf-IDF better. many better}
    \label{tab:git_visual_vs_sbert}
\end{table*}
